Extended Addressing Machines for PCF, with Explicit Substitutions

Addressing machines have been introduced as a formalism to construct models of the pure, untyped lambda-calculus. We extend the syntax of their programs by adding instructions for executing arithmetic operations on natural numbers, and introduce a reflection principle allowing certain machines to access their own address and perform recursive calls. We prove that the resulting extended addressing machines naturally model a weak call-by-name PCF with explicit substitutions. Finally, we show that they are also well-suited for representing regular PCF programs (closed terms) computing natural numbers.

==> include/conclusions.tex <==
% !TEX root = ../LICS.tex

We believe that the formalism of extended addressing machines introduced in this paper may contribute to the understanding of what can be considered as a sequential higher-order computation.
Indeed, EAMs are certainly sequential computational devices and higher-order computations are simply achieved by passing the address of a machine having a functional behaviour.
An objection that could be raised is that EAMs essentially incorporate the contents of the rewriting rules defining the operational semantics, whence they can be seen as a representation of \PCF{} operational semantics in disguise. We believe that this kind of criticism is due to an over-simplistic view. For instance, the fundamental difference in the way one handles variables and registers assignments in typing contexts shows that some machines can be hardly seen as representing subterms of the original \PCF{} program.
Another essential difference lies in the semantics of the recursion operator, which is achieved in the operational semantics through a (hidden) self-application, and in Scott-continuous models by computing the least fixed point of a continuous function. In the EAMs formalism the application mechanism is managed via a suitable assignment of addresses which by no means can be considered implicit in the operational semantics. Indeed the address table map is an arbitrary bijective function, constrained to some abstract conditions. As already discussed, there exist adequate address table maps having arbitrary computational complexity.
With this mechanism in place, the semantics of the fixed point operator is obtained by specifying a suitable EAM having its own address stored inside. 

In future works we wish to examine whether EAMs can be turned into a fully abstract model of \PCF{} by following the recipe presented in Section~\ref{ssec:Model}.
Besides being the key ingredient to obtain fully abstraction, Conjecture~\ref{conj1} suggests that one can bound the amount of addresses needed during the execution of a well-typed machine. By reinforcing this restriction, one could define ``finite state'' addressing machines that might represent an alternative way (w.r.t. game semantics) to compile higher-order, recursive programs with effects into FPGA fabrics~\cite{Ghica07,GhicaM00}.

We also plan to investigate whether the extra degree of freedom offered by the abstract nature of the address table map can be fruitfully applied to extend the computational capabilities of our machines (even in a well-typed setting), using the map $\Lookup(-)$ to import ``external resources''. Just to mention an example, one could consider the inclusion of a machine $\mach{Random(n)}$ that, when called via its address, returns a random integer number in the interval $[0, \ldots, n]$ (obeying some probability distribution). 
We think that it might be interesting to compare these AMs with the Probabilistic Krivine's Machines from~\cite{Ehrhard20}, and verify whether such a simple extension is sufficient to cope with the mathematical complexity needed to model Probabilistic \PCF .
Since probabilistic coherent spaces are fully abstract for Probabilistic \PCF, as shown by Ehrhard et al.~\cite{EhrhardPT18}, a full abstraction result for ``probabilistic'' addressing machines would simply follow from a finite definability property.
In other words, one should prove that any finite element of a probabilistic coherent space is definable by a machine of this kind.














==> include/model.tex <==
% !TEX root = ../LICS.tex
In this paper we mostly focused on the properties of the translation $\trans{-}{}{}$ from \PCF{} terms to EAMs, but we believe that extended addressing machines can be used to construct a fully abstract model of \PCF.
The Full Abstraction Problem for \PCF, originally proposed by Robin Milner in \cite{Milner77} (see also \cite{Plotkin77,BerryCL85,Curien92}), can be informally formulated as the problem of finding a ``natural'' model of PCF which is fully abstract w.r.t.\ the operational semantics. More precisely, two programs sharing the type $\alpha$ get the same denotation in a fully abstract model if and only if they are observationally indistinguishable when plugged in the same context $C[]$ of type $\alpha\to\tint$.
In the same paper, Milner proves that a fully abstract model can be obtained by a suitable completion of the ``term model" construction, and that this model is unique up to isomorphism (under some natural conditions).
The question is therefore whether it is possible to obtain this model using a direct ``semantic" construction. 

However, quoting from~\cite{AbramskyJM00},
\begin{quote} ``the problem is to understand what should be meant by a semantic characterization [\ldots] Our view is that the essential content of the problem, what makes it important, is that it calls for a semantic characterization of sequential, functional computation at higher-types''.
\end{quote}
A celebrated result is that fully abstract models of \PCF{} can be obtained by constructing suitable categories of games~\cite{AbramskyMJ94,AbramskyJM00,HylandO00}.
A fully abstract model based on realizability techniques was presented in \cite{MarzRS99}.
\subsection{PCF --- Observational Equivalence}

We briefly recall the definition of a fully abstract model of \PCF, and some basic results about observational equivalence.

\begin{definition}
\bsub
\item A \emph{\PCF{} context} $C[]$ is a \PCF{} term possibly containing occurrences of an algebraic variable, called \emph{hole} and denoted by [].
	Given a context $C[]$ and a \PCF{} term $P$, $C[P]$ stands for the \PCF{} term obtained by substituting $P$ for all occurrences of [] in $C[]$, possibly with capture of free variables.
	\item Given a context $C[]$, we write $C[] : \alpha\to\beta$ whenever $\vdash C[P] : \beta$ holds, for all $P$ of type $\alpha$.
\item Two \PCF{} programs $P,P'$ of type $\alpha$ are \emph{observationally equivalent}, written $P\equiv_{\textrm{obs}} P'$, whenever:
\[
	\forall C[] : \alpha \to\tint\,.\, [C[P] \redd\num n\iff C[P']\redd \num n]
\]
\item Two \PCF{} programs $P,P'$ of type $\alpha_1\to\cdots\to\alpha_k\to\tint$ are \emph{applicatively equivalent}, written $P\equiv_{\textrm{app}} P'$, when:
\[
	\forall Q_1 : \alpha_1,\dots,Q_k:\alpha_k \,.\, [P\vec Q \redd\num n\iff P'\vec Q \redd \num n]
\]
\esub
\end{definition}

The main difference between the observational equivalence in the untyped setting and the one for \PCF{} is that, in the latter, we observe the termination at ground type.
The following well-known result shows that the applicative and observational equivalence coincide on closed \PCF{} terms.

\begin{proposition}[Abramsky's equivalence]\label{prop:Abramsky} For all $\PCF$ programs $P,P'$ of type $\alpha$, we have
\[
	P\equiv_{\textrm{obs}} P' \iff P\equiv_{\textrm{app}} P'
\]
\end{proposition}


A model of \PCF{} is called \emph{fully abstract} whenever, for all \PCF{} programs $P,P'$ of type $\alpha$ the following holds:
\[
	\trans{P}{\tint}{} = \trans{P'}{\tint}{}\iff P\equiv_{\textrm{obs}} P'
\]
where `$=$' stands for the equality in the model under consideration.
The implication from left to right is called \emph{adequacy}, while the converse implication \emph{completeness}.
The models in \cite{AbramskyMJ94,AbramskyJM00,HylandO00,MarzRS99} are fully abstract in this sense.

\subsection{The Model Construction}\label{ssec:Model}

In this more speculative section, we show how it is possible to construct a model of \PCF{} based on extended abstract machines and explain the motivations that lead us to believe it might be fully abstract. 
Recall that a model of \PCF{} is given by a type-indexed collection of sets $(\cD_\alpha)_{\alpha\in\Types}$ with an associated application operation $(\cdot) : \cD_{\alpha\to\beta}\times\cD_\alpha\to\cD_\beta$. 
Intuitively, each $\cD_\alpha$ contains the interpretation $\trans{P}{}{}$ of any \PCF{} program $P$ having type $\alpha$.

\begin{definition}\bsub\item For all types $\alpha\in\Types$, define
	\[
	\cD_\alpha = \set{ a\in\Addrs \st~ \vdash \Lookinv a : \alpha}.
	\]
\item For all EAMs $\mM,\mN$ of type $\alpha$, define $\mM \equiv_\alpha \mN$ by induction on $\alpha$ as follows.
	\[
	\bar{lcl}
	\mM \equiv_\tint \mN &\iff& (\forall n\in\nat) [\mM \reddh \mach{n} \iff \mN \reddh \mach{n}] \\[1ex]
	\mM \equiv_{\alpha\to\beta} \mN&\iff&\forall a,b\in\cD_\alpha\,.\,[\Lookinv a \equiv_\alpha \Lookinv b \Rightarrow\\
	&&\qquad\qquad\quad\ \appT{\mM}{[a]} \equiv_\beta \appT{\mN}{[b]}]\\
	\ear
	\]
\item For $\alpha\in\Types$ and $a,b\in\cD_\alpha$, we let $a\simeq_\alpha b$ whenever $\Lookinv a\equiv_\alpha \Lookinv b$ holds.
\esub
\end{definition}

The candidate model for full abstraction is $(\cD_\alpha/\simeq_\alpha)_{\alpha\in\Types}$, where application is defined on the equivalence classes in the obvious way: $[a]_{\simeq_\alpha}\cdot [b]_{\simeq_\alpha} = [a\cdot b]_{\simeq_\alpha}$.
By Proposition~\ref{prop:Abramsky}, the full abstraction of the model follows if one can show that, for all \PCF{} programs $P,P'$ of type $\alpha$, $\trans{P}{\tint}{} \equiv_\alpha \trans{P'}{\tint}{}$ holds exactly when $P\equiv_{\textrm{obs}} P'$ does, where $\trans{-}{\tint}{}$ is the interpretation given in Definition~\ref{def:trans}.
The first step would be to prove the converse of Theorem~\ref{thm:main}, namely that, for a \PCF{} program $P$ of type $\tint$, $\trans{P}{}{}\reddh \mach{n}$ entails $P\redd \num n$. 
In order to establish this result, it is convenient to consider the small-step operational semantics of \PCF, since the big-step does not permit to handle non-terminating computations.
We believe that the adequacy of the model can be proved subsequently by exploiting syntactic logical relations as in \cite{Pitts97,Birkedal11,AhmedB11}.
Concerning the completeness of the model, we believe that it holds because of the following property.

\begin{conjecture}\label{conj1}
 Every element of $\cD_\alpha$ is definable by a \PCF{} program of type $\alpha$.
\end{conjecture}

In order to prove this statement one needs to exploit the fact that the typing mechanism harness the complexity of typable machines (independently from the chosen address table map $\Lookup$).
Indeed, while we have seen that there might exist EAMs $\mM$ that cannot be represented by a finite \PCF{} term (see Remark~\ref{rem:blackhole}), they cannot be typable since that would require an infinite derivation of $\vdash \mM : \alpha$, which is not allowed.
Thus, given an address $a\in\cD_\alpha$, it should be possible to construct by induction on a derivation of $\vdash a : \alpha$ a \PCF{} program $P$ of type $\alpha$ satisfying $\trans{P}{}{} \equiv_\alpha \Lookinv a$. The two machines might be different because useless instructions performed by $\Lookinv a$ will not give rise to any subterm of $P$, but their behaviours are observationally indistinguishable.

\begin{conjecture} $(\cD_\alpha/\simeq_\alpha)_{\alpha\in\Types}$  is fully abstract for \PCF.
\end{conjecture}
